A Density-Guided Temporal Attention Transformer for Indiscernible Object Counting in Underwater Video

Dense object counting or crowd counting has come a long way thanks to the recent development in the vision community. However, indiscernible object counting, which aims to count the number of targets that are blended with respect to their surroundings, has been a challenge. Image-based object counting datasets have been the mainstream of the current publicly available datasets. Therefore, we propose a large-scale dataset called YoutubeFish-35, which contains a total of 35 sequences of high-definition videos with high frame-per-second and more than 150,000 annotated center points across a selected variety of scenes. For benchmarking purposes, we select three mainstream methods for dense object counting and carefully evaluate them on the newly collected dataset. We propose TransVidCount, a new strong baseline that combines density and regression branches along the temporal domain in a unified framework and can effectively tackle indiscernible object counting with state-of-the-art performance on YoutubeFish-35 dataset.

==> response.tex <==
We appreciate the valuable feedback from the reviewers and have meticulously addressed the concerns raised. The key points can be summarized as follows:

1. Clarity on Contribution (Reviewers 2144, 3753):
- Our paper introduces two primary contributions: 
(1) The YoutubeFish5k dataset, a new video-based IOC dataset 
(2) The TransVidCnt baseline model, specifically designed to tackle the challenge of IOC with highly indiscernible targets.
- The model leverages temporal visual cues from density map supervision into the decoder, enhancing the prediction process. Our experiments demonstrate that temporal supervision significantly boosts performance in video-based IOC tasks.

2. Additional Dataset Insight (Reviewer 4B16):
- We acknowledge the importance of YoutubeFish-35 as the first publicly available video-based IOC dataset. Additional information highlighting the dataset's diversity will be included in the revised manuscript and on the dataset webpage to encourage broader benchmarking.

3. Benchmarking on Existing Dataset (Reviewers 4B16, 2144):
- Since there are no video-based IOC datasets, it motivates us to collect the YoutubeFish-35 dataset. And since it is a new benchmark, we ensure a fair comparison by adapting the original code [A, B] of the methods used, following the same fine-tuning process (in Table 2 of the paper).
- For the IOCfish5K dataset (image only), our 1-frame version of TransVidCount achieves slightly lower MAE (16.98), MSE(41.22), and the same NAE(0.38) compared with the numbers reported in the original IOCFormer[B] paper.

4. Clarity on Equation/Notation (Reviewers 4B16, 2144):
- We have revised the method section to enhance clarity, providing detailed explanations of the notations used in the equations.

5. Failure case and Error Analysis (Reviewers 2144): Due to the page limitations, additional images will be really difficult to fit, but we can use some red arrows and boxes to highlight the successful and failure cases (in Figure 3 of the paper) along with additional analyze in the experiment section.

We believe these revisions significantly strengthen our paper and address the concerns raised by the reviewers. We appreciate the opportunity to refine our work based on the constructive feedback provided.

[A] “An end-to-end transformer model for crowd localization,” D. Liang et al., ECCV2022.
[B] “Indiscernible object counting in underwater scenes,” G. Sun et al., CVPR2023.


=========================

We are grateful for the insightful feedback from the reviewers. Our revised manuscript incorporates these comments, and we outline the key revisions below:

1. Clarity on Contribution (Reviewers 2144, 3753):

We clarify our two primary contributions:
(1) YoutubeFish5k dataset: An innovative video-based IOC dataset.
(2)TransVidCnt baseline model: Designed specifically for IOC tasks with minimally distinguishable targets. The model uniquely integrates temporal visual cues from density maps into the decoder, enhancing prediction accuracy. Our empirical results substantiate the significant performance improvement in video-based IOC tasks due to this temporal supervision.

2. Additional Dataset Insight (Reviewer 4B16):

We acknowledge the pioneering nature of the YoutubeFish-35 dataset as the inaugural publicly available video-based IOC dataset. The revised manuscript will include enhanced details about the dataset's diversity, and these insights will also be reflected on our dataset webpage to facilitate broader benchmarking.

3. Benchmarking on Existing Dataset (Reviewers 4B16, 2144):

Given the absence of comparable video-based IOC datasets, our YoutubeFish-35 dataset serves as a new benchmark. We ensure fair comparisons by adapting the original code [A, B] of referenced methods and following identical fine-tuning processes (as detailed in Table 2 of our paper).
Regarding the IOCfish5K dataset (image-only), our single-frame TransVidCount model achieves comparable MAE, MSE, and NAE (16.98/41.02/0.38) compared to the original IOCFormer[B] paper (17.12/41.25/0.38), emphasizing the robustness of our approach.

4. Clarity on Equation/Notation (Reviewers 4B16, 2144):

The manuscript's method section has been revised for enhanced clarity. We provide detailed explanations of the notations used in the equations to ensure comprehension.

5. Failure Case and Error Analysis (Reviewer 2144):

Due to page constraints, including additional images for failure case analysis is challenging. However, we will utilize red arrows and boxes in Figure 3 to highlight successful and unsuccessful instances, accompanied by a detailed analysis in the experiment section.
We trust that these revisions substantially strengthen our submission and adequately address the reviewers' concerns. We value the opportunity to refine our work based on this constructive feedback.

References:
[A] D. Liang et al., “An end-to-end transformer model for crowd localization,” ECCV 2022.
[B] G. Sun et al., “Indiscernible object counting in underwater scenes,” CVPR 2023.
